Service Function Chaining Simplified

Middleboxes have become a vital part of modern networks by providing service functions such as content filtering, load balancing and optimization of network traffic. An ordered sequence of middleboxes composing a logical service is called service chain. Service Function Chaining (SFC) enables us to define these service chains. Recent optimization models of SFCs assume that the functionality of a middlebox is provided by a single software appliance, commonly known as Virtual Network Function (VNF). This assumption limits SFCs to the throughput of an individual VNF and resources of a physical machine hosting the VNF instance. Moreover, typical service providers offer VNFs with heterogeneous throughput and resource configurations. Thus, deploying a service chain with custom throughput can become a tedious process of stitching heterogeneous VNF instances. In this paper, we describe how we can overcome these limitations without worrying about underlying VNF configurations and resource constraints. This prospect is achieved by distributed deploying multiple VNF instances providing the functionality of a middlebox and modeling the optimal deployment of a service chain as a mixed integer programming problem. The proposed model optimizes host and bandwidth resources allocation, and determines the optimal placement of VNF instances, while balancing workload and routing traffic among these VNF instances. We show that this problem is NP-Hard and propose a heuristic solution called Kariz. Kariz utilizes a tuning parameter to control the trade-off between speed and accuracy of the solution. Finally, our solution is evaluated using simulations in data-center networks.

==> charts/all-util.tex <==
\begin{figure*}
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=0.32\textwidth]{charts/legend.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/all-bandwidth-util.eps}
        \caption{Bandwidth Utilization}
        \label{fig:all-bandwidth-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/all-cpu-util.eps}
        \caption{CPU Utilization}
        \label{fig:all-cpu-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/all-vnf-util.eps}
        \caption{VNF Utilization}
        \label{fig:all-vnf-util}
    \end{subfigure}
    \caption{Resources Utilization}
    \label{fig:all-util}
\end{figure*}

==> charts/bandwidth-util.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/kariz-Bandwidth-util.eps}
        \caption{Kariz Bandwidth Utilization}
        \label{fig:kariz-bandwidth-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/optimal-Bandwidth-util.eps}
        \caption{MIP Bandwidth Utilizaiton}
        \label{fig:mip-bandwidth-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/Bandwidth-util.eps}
        \caption{Comparison of Bandwidth Utilization}
        \label{fig:bandwidth-comp-util}
    \end{subfigure}
    \caption{Bandwidth Utilization}
    \label{fig:bandwidth-util}
\end{figure*}

==> charts/cpu-util.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/kariz-CPU-util.eps}
        \caption{Kariz CPU Utilization}
        \label{fig:cpu-kariz-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/optimal-CPU-util.eps}
        \caption{MIP CPU Utilizaiton}
        \label{fig:cpu-mip-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/CPU-util.eps}
        \caption{Comparison of CPU Utilization}
        \label{fig:cpu-comp-util}
    \end{subfigure}
    \caption{CPU Utilization}
    \label{fig:cpu-util}
\end{figure*}

==> charts/vnf-util.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/kariz-VNF-util.eps}
        \caption{Kariz VNF Utilization}
        \label{fig:kariz-VNF-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/optimal-VNF-util.eps}
        \caption{MIP VNF Utilizaiton}
        \label{fig:mip-VNF-util}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{charts/util/VNF-util.eps}
        \caption{Comparison of VNF Utilization}
        \label{fig:vnf-comp-util}
    \end{subfigure}
    \caption{VNF Utilization}
    \label{fig:vnf-util}
\end{figure*}

==> equations/bandwidthDemandCons.tex <==
\begin{equation}
\small
    \begin{aligned}
        &\forall \overline{v} \in \overline{V}:
        \\
            &\sum_{v \in \mathcal{N}_{\overline{v}}} {
                \sum_{(u,v) \in \mathcal{L}^{in}_{v}} {
                    \sum_{n \in N_V} {
                        \sum_{(m,n) \in L_{n}, m < n} {
                            y_{vn}(
                                x_{uv}^{mn} + x_{uv}^{nm}
                            )
                        }
                    }
                }
            }
            = y_{vn} \overline{b}
        \\
            &\sum_{v \in \mathcal{N}_{\overline{v}}} {
                \sum_{(v,u) \in \mathcal{L}^{out}_{v}} {
                    \sum_{n \in N_V} {
                        \sum_{(m,n) \in L_{n}, m < n} {
                            y_{vn}(
                                x_{vu}^{mn} + x_{vu}^{nm}
                            )
                        }
                    }
                }
            }
            = y_{vn} \overline{b}
    \end{aligned}
    \label{equation:bandwidthDemandCons}
\end{equation}

==> equations/dynamicProgramming.tex <==
\begin{equation}
\hspace*{-0.282cm}
\small
    a(i,\omega)=
    \begin{dcases*}
        g_i(-\omega)    & if $i=1$ \\
        \min_{\delta}{
            \big(
            g_i(\delta) + a(i-1, \omega + \delta)
            \big)
        }              & $i=2, \ldots, |L(\overline{v})|$
    \end{dcases*}
    \label{equation:dynamicProgramming}
\end{equation}

==> equations/flowConst.tex <==
\begin{equation}
\small
    \forall u \in \mathcal{N}:
        \sum_{(u,v) \in \mathcal{L}^{out}_u} {
            \hat{x}_{uv}
        }
        -
        \sum_{(v,u) \in \mathcal{L}^{in}_u} {
            \hat{x}_{vu}
        }
        =
        \begin{cases}
            \overline{b}  &  \mbox{if } u \in \{\overline{i}\}\\
            -\overline{b} &  \mbox{if } u \in \{\overline{j}\}\\
            0             &  \mbox{otherwise}
        \end{cases}
    \label{equation:flowConst}
\end{equation}

==> equations/linkAsnCons.tex <==
\begin{equation}
\small
    \begin{aligned}
        &\forall u \in \mathcal{N}:
            \forall (u,v) \in \mathcal{L}^{out}_{u}:
                \forall m \in N:
                \\
                    &\sum_{(m,n) \in L_m} {(
                        x_{uv}^{mn} - x_{uv}^{nm}
                    )}
                    =
                    z_{uv}^{um} - z_{uv}^{vm}
    \end{aligned}
    \label{equation:linkAsnCons}
\end{equation}

==> equations/loopFreeConst.tex <==
\begin{equation}
    \small
    \forall u \in \mathcal{N}:
        \forall (u,v) \in \mathcal{L}^{out}_u:
            \forall m \in N:
                \frac{1}{\Gamma} \hat{x}_{uv} + 
                y_{um} + y_{vm}
                \leq
                2
    \label{equation:loopFreeConst}
\end{equation}

==> equations/nodeAsnConst.tex <==
\begin{equation}
\small
    \forall u \in \mathcal{N}:
        \sum_{m \in N} {
            y_{um}
            \leq
            1
        }
    \label{equation:nodeAsnConst}
\end{equation}

==> equations/nodeAsnCost.tex <==
\begin{equation}
    \mathscr{C}_{N} =
        \sum_{v \in \mathcal{N}} {
            \sum_{n \in N}{
                \sum_{r \in R} {
                    \alpha_r y_{vn} d_{vr}
                }
            }
        }
    \label{equation:nodeAsnCost}
\end{equation}

==> equations/pivotCost.tex <==
\begin{equation}
    
    \label{equation:pivotCost}
\end{equation}

==> equations/slackVariable1.tex <==
\begin{equation}
\small
\begin{aligned}
    &\forall n \in N:
        \forall (m,n) \in L_n, m < n:
            \forall v \in \mathcal{N}:
                \forall (u,v) \in \mathcal{L}_{v}^{in}: \\
                    &z_{uv}^{mn} = 
                        \begin{cases}
                            x_{uv}^{mn} &  \mbox{if } y_{vn} = 1\\
                            0           &  \mbox{if } y_{vn} = 0
                        \end{cases}
\end{aligned}
\label{equation:slackVariable1}
\end{equation}

==> equations/slackVariable2.tex <==
\begin{equation}
\small
\begin{aligned}
    &\forall n \in N:
        \forall (m,n) \in L_n, m < n:
            \forall v \in \mathcal{N}:
                \forall (v, u) \in \mathcal{L}_{v}^{out}: \\
                    &\hat{z}_{vu}^{mn} = 
                        \begin{cases}
                            x_{vu}^{mn} &   \mbox{if } y_{vn} = 1\\
                            0           &   \mbox{if } y_{vn} = 0
                        \end{cases}
\end{aligned}
\label{equation:slackVariable2}
\end{equation}

==> equations/slackVariablesConst.tex <==
\begin{equation}
\small
\label{equation:slackVariablesConst}
    \begin{aligned}
        z   &\leq   \Gamma y
        &,
        z   &\geq   0                \\
        z   &\leq   x
        &,
        z   &\geq   x - (1-y) \Gamma
    \end{aligned}
\end{equation}

==> equations/throughputConst.tex <==
\begin{equation}
\small
    \begin{aligned}
        &\forall v \in \mathcal{N}:
            \forall n \in N:
            \\
                &\sum_{(u,v) \in \mathcal{L}^{in}_{v}}{
                    \sum_{(m,n) \in L_{n}, m < n} {
                        y_{vn} (
                            x^{mn}_{uv} + x^{nm}_{uv}
                        )
                    }
                }
                \leq
                q_v
            \\
                &\sum_{(v,u) \in \mathcal{L}^{out}_{v}}{
                    \sum_{(m,n) \in L_{n}, m < n} {
                        y_{vn} (
                            x^{mn}_{vu} + x^{nm}_{vu}
                        )
                    }
                }
                \leq
                q_v
    \end{aligned}
    \label{equation:throughputConst}
\end{equation}

==> equations/virtualVNFPerfConst.tex <==
\begin{equation}
\small
    \forall \overline{v} \in \overline{V}:
        \sum_{v \in \mathcal{V}_{\overline{v}}} {
            \sum_{n \in N_V} {
                y_{vn}q_v
                \geq
                \overline{b}
            }
        }
    \label{equation:virtualVNFPerfConst}
\end{equation}

==> equations/xhat.tex <==
\begin{equation}
\small
    \hat{x}_{uv}^{mn} = 
    \begin{cases}
        1   &  \mbox{if } x_{uv}^{mn} > 0, \\
        0   &  \mbox{if } x_{uv}^{mn} = 0
    \end{cases}
    \label{equation:xhat}
\end{equation}

==> equations/z.tex <==
\begin{equation}
\small
    z_{uv}^{wm} = 
        \begin{cases}
            \hat{x}_{uv} &  \mbox{if } y_{wm} = 1\\
            0            &  \mbox{if } y_{wm} = 0
        \end{cases}
\label{equation:z}
\end{equation}

==> equations/zhat.tex <==
\begin{equation}
\small
    \hat{z}_{vu}^{mn} = 
        \begin{cases}
            x_{vu}^{mn} &   \mbox{if } y_{vn} = 1\\
            0           &   \mbox{if } y_{vn} = 0
        \end{cases}
\label{equation:zhat}
\end{equation}

==> figures/layers/layers.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/layers/network.eps}
        \caption{Substrate Network}
        \label{fig:layersNetwork}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/layers/request.eps}
        \caption{Service Chain Request}
        \label{fig:layersSCR}
    \end{subfigure}
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/layers/initial.eps}
        \caption{Layers}
        \label{fig:layersInitial}
    \end{subfigure}
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/layers/with-flows.eps}
        \caption{Layers with Traffic}
        \label{fig:layersWithFlow}
    \end{subfigure}
    \hfill
    \caption{Layers}
    \label{fig:layers}
\end{figure*}

==> figures/notation.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/notation/network.eps}
        \caption{Substrate Network}
        \label{fig:networkNot}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/notation/request.eps}
        \caption{Service Chain Request}
        \label{fig:serviceChainRequestNot}
    \end{subfigure}
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/notation/embedded.eps}
        \caption{Network Flow Decision Var.}
        \label{fig:embeddedNot}
    \end{subfigure}
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/notation/logical.eps}
        \caption{VNF Replicas Decision Var.}
        \label{fig:logicalRepNot}
    \end{subfigure}
    \hfill
    \caption{Notation and Decision Variables}
    \label{fig:notation}
\end{figure*}

==> figures/split.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/split/sample.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=0.39\textwidth]{figures/split/description.eps}
    \end{subfigure}
    \caption{Per-flow Traffic Splitting}
    \label{fig:split}
\vspace{-0.6cm}
\end{figure}

==> figures/transformation.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/transformation/description.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/transformation/serviceChainRequest.eps}
        \caption{Service Chain Request}
        \label{fig:serviceChainRequest}
    \end{subfigure}
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/transformation/nodeSplitting.eps}
        \caption{Virtual VNF Splitting}
        \label{fig:nodeSplitting}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/transformation/linkSplitting.eps}
        \caption{Virtual Link Splitting}
        \label{fig:linkSplitting}
    \end{subfigure}
    \caption{Transformation}
    \label{fig:transformation}
\end{figure*}

==> sections/acknowledgements.tex <==
\section{Acknowledgement}
This work was supported by the Natural Science and Engineering Council of Canada (NSERC) under the Smart Applications on Virtual Infrastructure (SAVI) Research Network. Further, this work benefited from the use of the CrySP RIPPLE Facility at the
University of Waterloo.

==> sections/relatedWorks/splitMerge.tex <==
Splite/Merge\cite{splitMerge} proposes a system for elastic deployment of VNFs. The authors specifically addressed challenges of VNF state management and traffic routing management. However, their solution requires huge modification in current VNFs to be deployable in their framework.

\textbf{More Details:} The authors to address state management, they classified state of a VM hosting a VNF to internal, partitioned, and coherent. The internal state is the VM state is related to a single replica. The partitioned state is related to a subset of input, and should be modified by the replica which processes this input. Coherent state is accessed by multiple state machine replicas and should be synchronized. To route the traffic to correct replicas, the SDN capabilities supported in open vSwitch is leveraged.


==> tables/motivation.tex <==
\begin{table}
    \caption{VNF Performances}
    \vspace{-0.6cm}
    \scriptsize
    \begin{tabular}{c||c|c|c|c}
        Virtual VNF     & VNF       & Perf.     & Throughput    & CPU Demand    \\ \hline
        $VNF_1$         & $u_1$     & 30        & 240           & 8             \\
                        & $u_2$     & 15        & 120           & 4             \\ \hdashline
        $VNF_2$         & $v_1$     & 40        & 160           & 4             \\
                        & $v_2$     & 20        & 80            & 2             \\ \hdashline
        $VNF_3$         & $w_1$     & 15        & 80            & 2             \\
    \end{tabular}
    \label{table:sample}
\end{table}


==> tables/notation.tex <==
\begin{table}
\scriptsize
    \caption{Notation}
    \begin{tabular}{l*{2}{l}}
        Symbol                          & Meaning                                                       \\
        \hline                                                      
        $R$                             & Resources 	                                                \\
        $r$                             & A resource                                                    \\
        $V$                             & VNFs                                                          \\
        $v$                             & A VNF                                                         \\
        $p_v$                           & Performance of VNF $v$                                        \\
        $q_v$                           & Throughput of VNF $v$                                         \\
        $d_{vr}$                        & Demand of VNF $v$ for resource $r$                            \\
        $G$                             & Substrate network                                             \\
        $N$                             & Substrate nodes                                               \\
        $N_V$                           & Substrate nodes in which VNFs are installed                   \\
        $n$                             & A substrate node                                              \\
        $c_{nr}$                        & Residual capacity of node $n$ for resource $r$                \\
        $L$                             & Substrate Links                                               \\
        $L_n$                           & Incident substrate links on node $n$                          \\
        $(m,n)$                         & A substrate link between nodes $m$ and $n$                    \\
        $c_{mn}$                        & Residual bandwidth capacity of link $(m,n)$                   \\
        $\overline{G}$                  & Service chain request                                         \\
        $\overline{N}$                  & Virtual nodes                                                 \\
        $\overline{src}$                & Source (virtual node) of traffic of service chain request's   \\
        $src$                           & Source (substrate node) of traffic of service chain request's \\
        $\overline{trg}$                & Target (virtual node) of traffic of service chain request's   \\
        $trg$                           & Target (substrate node) of traffic of service chain request's \\
        $\overline{V}$                  & Virtual VNFs                                                  \\
        $\overline{v}$                  & A virtual VNF                                                 \\
        % $\overline{p}_{\overline{v}}$   & Performance demand of virtual VNF $v$                         \\
        $\overline{L}$                  & Virtual Links                                                 \\
        $\overline{b}$                  & Bandwidth demand of service chain                             \\
        $\mathcal{N}$                   & Meta nodes                                                    \\
        $\mathcal{N}_{\overline{v}}$    & Meta context of virtual VNF $v$                               \\
        $\mathcal{L}$                   & Meta Links                                                    \\
        $\mathcal{L}_{v}$               & Incident meta links on meta node $v$                          \\
        $\mathcal{L}^{in}_{v}$          & Incoming incident meta links on meta node $v$                 \\
        $\mathcal{L}^{out}_{v}$         & Outgoing incident meta links on meta node $v$                 \\
        $y_{vn}$                        & Assignment of meta node $v$ to substrate node $n$             \\
        $x_{uv}^{mn}$                   & Flow of meta link $(u,v)$ on substrate link $(m,n)$           \\
        $\alpha_r$                      & Relative importance of resource $r$                           \\
        $\alpha_{BW}$                   & Relative importance of bandwidth resources                    \\
        \hline
    \end{tabular}
    \label{table:notation}
\end{table}

